MALS discovery of a rare HI 21-cm absorber at $z\sim1.35$: origin of the absorbing gas in powerful AGN

We report a new, rare detection of HI 21-cm absorption associated with a quasar (only six known at $1<z<2$) here towards J2339-5523 at $z_{em}$ = 1.3531, discovered through the MeerKAT Absorption Line Survey (MALS). The absorption profile is broad ($\sim 400$ km/s), and the peak is redshifted by $\sim 200$ km/s, from $z_{em}$. Interestingly, optical/FUV spectra of the quasar from Magellan-MIKE/HST-COS spectrographs do not show any absorption features associated with the 21-cm absorption. This is despite the coincident presence of the optical quasar and the radio `core' inferred from a flat spectrum component of flux density $\sim 65$ mJy at high frequencies ($>5$ GHz). The simplest explanation would be that no large HI column (N(HI)$>10^{17}$ cm$^{-2}$) is present towards the radio `core' and the optical AGN. Based on the joint optical and radio analysis of a heterogeneous sample of 16 quasars ($z_{median}$ = 0.7) and 15 radio galaxies ($z_{median}$ = 0.3) with HI 21-cm absorption detection and matched in 1.4 GHz luminosity (L$_{\rm 1.4\,GHz}$), a consistent picture emerges where quasars are primarily tracing the gas in the inner circumnuclear disk and cocoon created by the jet-ISM interaction. These exhibit L$_{1.4\,\rm GHz}$ - $\Delta V_{\rm null}$ correlation, and frequent mismatch between the radio and optical spectral lines. The radio galaxies show no such correlation and likely trace the gas from the cocoon and the galaxy-wide ISM outside the photoionization cone. The analysis presented here demonstrates the potential of radio spectroscopic observations to reveal the origin of the absorbing gas associated with AGN that may be missed in optical observations.

==> table3_AA.tex <==
\begin{sidewaystable*}
\tabcolsep=4pt
\caption{Quasars with \hi\ 21-cm absorption from literature. \label{tab:litqso}.}
\centering
\begin{tabular}{lccccccccccllc}
\hline\hline             
Source name  & $z_{em}$(opt)  & $z_{abs}$ & V$_{null, B}$ & V$_{null, R}$ & S$_{1.4GHz}$ & $\alpha$ & $\log \rm L_{1.4 GHz}^*$ &  S$_{21-cm}$ & $\int \tau\ dv$   & 21-cm Ref. & LAS & LLS & Ref.\\
   &   &   & (\kms\,) & (\kms\,) & (mJy) &  & (\,W\,Hz$^{-1}$) &  (mJy) & (\kms\,)  &  & (arcsec) & (kpc) & \\
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14)\\
\hline
J000557.17$+$382015.2 & 0.229 & 0.229 & -45.4 & 48.2 & 572.7 & -0.03 $\pm$ 0.10 & 25.9 & 547.3 & 1.943 $\pm$ 0.057 & 1 & 0.043 & 0.162 & 1, 13 \\
J011137.31$+$390627.9 & 0.67 & 0.668 & -69.9 & 137.0 & 429.0 & 2.09 $\pm$ 0.05 & 26.3 & 180.0 & 46 $\pm$ 7 & 2 & 0.005 & 0.036 & 19\\
J050321.20$+$020304.6 & 0.5834 & 0.5848 & -98.7 & 57.7 & 2245.1 & 1.07 $\pm$ 0.04 & 27.1 & 1600.0 & 3.4 $\pm$ 0.4 & 2 & 0.011 & 0.073 & 19 \\
J061048.87$+$724853.2 & 3.52965 & 3.52983 & -643.0 & 639.0 & 1041.6 & -0.37 $\pm$ 0.07 & 28.7 & 1790.2 & 4.69 $\pm$ 0.15 & 3 & 0.050 & 0.373 & 3, 15\\
J080133.56$+$141443.0 & 1.1946 & 1.1929 & -198.4 & 494.9 & 2734.6 & -1.10 $\pm$ 0.11 & 28.4 & 5690.0 & 2.47$\pm$0.05 & 4 &  4.0 & 33.0 & 4\\
J090933.50$+$425346.5 & 0.67 & 0.67 & -259.8 & 273.5 & 4234.2 & -0.80 $\pm$ 0.10 & 27.9 & 6218.1 & 0.68 & 5,6 & 9.2 & 64.5 & 19 \\
J120321.94$+$041419.0 & 1.22429 & 1.20888 & -105.8 & 679.1 & 1146.6 & -0.65 $\pm$ 0.11 & 27.9 & 1675.2 & 2.52 $\pm$ 0.12 & 7 & 0.075 & 0.458 & 7, 16 \\
J124823.89$-$195918.8 & 1.275 & 1.275 & -713.3 & 250.8 & 5136.1 & -0.59 $\pm$ 0.04 & 28.6 & 8302.2 & 4.542 $\pm$ 0.043 & 7 & 0.040 & 0.230 & 20 \\
J145844.79$+$372021.5 & 0.33324 & 0.33316 & -41.3 & 37.0 & 215.1 & -0.02 $\pm$ 0.03 & 25.8 & 148.4 & 3.834 $\pm$ 0.079 & 1 & $<0.01$ & $<0.0495$ & 1, 14\\
J150609.53$+$373051.1 & 0.674 & 0.673 & -327.8 & 74.0 & 937.6 & 0.05 $\pm$ 0.10 & 27.1 & 1040.0 & 27.20 $\pm$ 0.04 & 8,9 &  0.055 & 0.387 & 9, 17\\
J154015.23$-$145341.5 & 2.104 & 2.1139 & -176.1 & 90.0 & 203.7 & -0.69 $\pm$ 0.04 & 27.7 & 652.0 & 11.30 $\pm$ 0.07 & 10 & $>$0.050  & $>$0.425 & 10, 18 \\
J154508.52$+$475154.6 & 1.277 & 1.2797$^{\dag}$ & -334.5 & 204.0 & 685.7 & -0.36 $\pm$ 0.09 & 27.6 & 861.5 & 9.56 $\pm$ 0.36 & 1 & 0.060 & 0.516 & 11\\
J181536.79$+$612711.6 & 0.601 & 0.594 & -118.6 & 166.0 & 849.3 & -0.48 $\pm$ 0.08 & 27.0 & 971.6 & 2.39 & 6 & 0.01 & 0.068 & 19 \\
J195542.73$+$513148.5 & 1.223 & 1.2206 & -62.5 & 42.3 & 1588.1 & 0.01 $\pm$ 0.09 & 27.8 & 1254.1 & 0.716 $\pm$ 0.037 & 12 & $>0.050^{\dag\dag}$ & $>0.4275^{\dag\dag}$ & 12\\
J233913.22$-$552350.4 & 1.353 & 1.355 & -86.4 & 310.8 & 184.2 & -0.71 $\pm$ 0.01 & 27.2 & 336.0 & 3.7 $\pm$ 0.2 & ... & $<$0.6 & $<5.2$ & ... \\
J225503.88$+$131333.9 & 0.543 & 0.543 & -101.8 & 116.9 & 2706.8 & -0.83 $\pm$ 0.11 & 27.5 & 3725.5 & 0.23 & 6 & 2.6 & 16.5 & 19\\
\hline
\hline
\end{tabular}
\tablebib{
(1) \cite{Aditya18}; (2) \cite{Carilli98}; (3) \cite{Aditya21}; (4) \cite{Ishwara03}; (5) \cite{Pihlstrom99}; (6) \cite{Vermeulen03}; (7) \cite{Aditya18gps}; (8) \cite{Carilli92}; (9) \cite{Kanekar08}; (10) \cite{Gupta21hz}; (11) \cite{Malkin2018}; (12) \cite{Aditya17}; (13) \cite{Fey00}; (14) \cite{Helmboldt07}; (15) \cite{Britzen07}; (16) \cite{Liu07}; (17) \cite{Polatidis95}; (18) \cite{Gupta22m1540}; (19) \cite{Gupta06}; (20)\cite{Sokolovsky11}.
}
\tablefoot{
\small{
    Column\,1: Source name (J2000); Column\,2: Optical redshift; Column\,3: Peak \hi\ 21-cm absorption redshift; Column\,4 - 5: Velocity to the bluer and redder side of the peak, respectively, where the optical depth goes below the spectrum sensitivity; Column\,6: Flux density at 1.4 GHz; Column\,7: Spectral index and its associated uncertainty; Column\,8: Radio luminosity at 1.4\,GHz; Column\,9: Flux density at the redhsifted 21-cm line frequency; Column\,10: Total velocity integrated optical depth; Column\,11: \hi\ 21-cm absorption reference; Column\,12: Largest Angular Size in arcsec, and Column\,13: Largest Linear Size in kpc; Column\,14: Reference for LAS and LLS.\\}
    
    \footnotesize{$^{\dag}$ centroid of two Gaussian components of similar amplitudes\\
    $^{\dag\dag}$ size of the radio-core against which the absorption was observed (see \cite{Aditya17} for more details)\\
    $^*$ Derived using 1.4\,GHz (NVSS) and 4.85\,GHz flux densities from NED. In four cases, the spectral turnover falls between 1.4\,GHz and 4.85\,GHz, or 4.85\,GHz measurement is unavailable or dubious.  For these measurements at 1.4~GHz and at a lower frequency were used.\\}    
}
\end{sidewaystable*}

==> table4_AA.tex <==
\begin{table*}[h]
\tabcolsep=4pt
\centering
\caption{Rest equivalent width (W$_r$ in $\AA$) estimates from optical spectra. \label{tab:EW}}
\begin{tabular}{lcccccc}
\hline \hline
Source name  & $z_{em}$(opt) &  Reference &$\lambda_{obs}$ ($\AA$) & $\lambda_{rest}$ ($\AA$) & Line & W$_r$ ($\AA$)\\
%{MgII2796} &  {MgII2796} & {MgI2853} & {MgI2853} & {CIV1549} & {CIV1549} & {SiIV1394} & {SiIV1394} \\
(1) & (2) & (3) & (4) & (5) & (6) & (7)\\
\hline
    \multicolumn{7}{c}{} \\
    \multicolumn{7}{c}{\large Quasars} \\
    \multicolumn{7}{c}{} \\
\hline
J0111$+$3906$^\dag$ & 0.67 & 1 & ... & 2694$-$5567 & MgII2796, MgI2853 & $<$4.633, $<$4.633 \\
J0801$+$1414 & 1.1946 & 2 & 3800$-$9200 & 1731$-$4192 &  MgII2796, MgI2853 & 1.865, 1.245\\
J0909$+$4253 & 0.67 & 2 & 3800$-$9200 & 2275$-$5509 &  MgII2796, MgI2853 & $<$0.744, $<$0.744 \\
J1203$+$0414 & 1.22429 & 2 & 3800$-$9200 & 1708$-$4136 & MgII2796, MgI2853 & $<$0.270, $<$0.266\\
J1458$+$3720 & 0.33324 & 2 & 3800$-$9200 & 2852$-$6900 & ... & ...\\
%J1955$+$5131 & 1.223 & 1 & 1720$-$4426 & 773$-$1991 & CIV1549, SiIV1394 & $<$0.026, 0.657\\
J1955$+$5131 & 1.223 & 3 & 5502$-$9841 & 2475$-$4427 & MgII2796, MgI2853 & $<$0.316, $<$0.139 \\
\hline
    \multicolumn{7}{c}{} \\
    \multicolumn{7}{c}{\large Radio galaxies } \\
    \multicolumn{7}{c}{} \\
\hline
J0834$+$5534 & 0.242   & 2 & 3800$-$9200 & 3059$-$7407 & NaI5891 & 2.0 \\
J0901$+$2901 & 0.194   & 2 & 3800$-$9200 & 3182$-$7705 & CaII3934, NaI5891 & 6.8, 1.5  \\
J1400$+$6210 & 0.431   & 2 & 3800$-$9200 & 2655$-$6429 & CaII3934, NaI5891 &  5.9, 2.7 \\
%J2316$+$0405 & 0.2199  & 4 & 3500$-$8044 & 2869$-$6594 & CaI4228, CaII3935, NaI5892 &  Poor resolution spectrum  \\
J2355$+$4950$^\dag$ & 0.2379  & 1 & ...     & 3036$-$7962 & CaII3934, NaI5891 & 7.8, 3.8 \\
J1247$+$4900 & 0.20691 & 2 & 3800$-$9200 & 3148$-$7623 & CaII3934        & 6.0   \\
\hline
\end{tabular}
\tablebib{(1) \cite{Lawrence96}; (2) \cite{SDSSDR6}; (3) \cite{Torrealba12}.}
\tablefoot{
\small{
    Column\,1: Source name (J2000); Column\,2: Optical redshift; Column\,3: Optical spectrum reference; Column\,4: $\lambda$ range (in $\AA$) covered in the observed frame; Column\,5: $\lambda$ range (in $\AA$) covered in the rest frame; Column\,6: Metal lines covered by the wavelength range; Column\,7: Rest equivalent width (W$_r$) estimates or upper limits.\\}
    
    \footnotesize{$^{\dag}$ the available optical spectrum is in the rest frame.}
}
\end{table*}

==> table5_AA.tex <==
\begin{sidewaystable*}
\tabcolsep=4pt
\caption{Radio galaxy sample with \hi\ 21-cm absorption from literature. \label{tab:litgals}}
\centering
\begin{tabular}{lcccccccccllc}
\hline\hline             
Source name  & $z_{em}$(opt)  & $z_{abs}$ & V$_{null, B}^{\dag}$ & V$_{null, R}^{\dag}$ & S$_{1.4\rm GHz}$ & $\log \rm L_{1.4 GHz}$ &  S$_{21-cm}$ & $\int \tau\ dv$   & 21-cm Ref. & LAS & LLS & Ref.\\
  &  & & (\kms\,) & (\kms\,) & (mJy) & (\,W\,Hz$^{-1}$) &  (mJy) & (\kms\,) &  & (arcsec) & (kpc) & \\ 
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
\hline
J0025$-$2602 & 0.322 & 0.322  & $-$349  & 115     & 8.753 & 27.5 &  8.17  & 1.33  & 1 & 0.65  & 3.02  & 3 \\
J0141$+$1353 & 0.621 & 0.620  & $-$225  & $-$141  & 2.74  & 27.7 &  3.78  & 0.64  & 1 & 0.99  & 6.71  & 3 \\
J0431$+$2037 & 0.219 & 0.219  & $-$54   & 92      & 3.756 & 26.7 &  4.56  & 2.00  & 1 & 0.29  & 1.02  & 3 \\
J0834$+$5534 & 0.242 & 0.240  & $-$672  & $-$152  & 8.283 & 27.1 &  7.22  & 0.61  & 1 & 11.0  & 41.4  & 3 \\
J0901$+$2901 & 0.194 & 0.194  & $-$161  & 131     & 2.004 & 26.3 &  2.006 & 0.06  & 1 & 5.7   & 18.2  & 3 \\
J1206$+$6413 & 0.371 & 0.372  & 130     & 407     & 3.720 & 27.3 &  3.34  & 1.13  & 1 & 1.3   & 6.6   & 3 \\
J1326$+$3154 & 0.370 & 0.368  & $-$760  & $-$218  & 4.862 & 27.3 &  5.405 & 0.41  & 1 & 0.056 & 0.285 & 3 \\
J1357$+$4354 & 0.646 & 0.645  & $-$585  & 266     & 0.704 & 27.0 &  0.50  & 19.53 & 1 & 0.017 & 0.117 & 3 \\
J1400$+$6210 & 0.431 & 0.430  & $-$470  & $-$65   & 4.308 & 27.5 &  5.47  & 1.10  & 1 & 0.065 & 0.362 & 3 \\
J1821$+$3942 & 0.798 & 0.793  & $-$923  & $-$672  & 3.507 & 28.0 &  5.17  & 0.96  & 1 & 0.47  & 3.53  & 3 \\
J1944$+$5448 & 0.263 & 0.257  & $-$1782 & $-$1075 & 1.754 & 26.6 &  1.95  & 2.88  & 1 & 0.040 & 0.161 & 3 \\
J2052$+$3635 & 0.355 & 0.355  & $-$168  & $-$72   & 5.144 & 27.2 &  4.5   & 4.24  & 1 & 0.060 & 0.297 & 3 \\
J2316$+$0405 & 0.220 & 0.219  & $-$405  & $-$803  & 4.676 & 26.8 &  4.97  & 0.43  & 1 & 1.86  & 6.55  & 4 \\
J2355$+$4950 & 0.238 & 0.238  & $-$111  & 150     & 2.306 & 26.6 &  2.25  & 1.66  & 1 & 0.069 & 0.256 & 3 \\
J1247$+$4900 & 0.207 & 0.207  & $-$757  & 61      & 1.140 & 26.1 &  1.226 & 0.46  & 2 & 2.64  & 5.4   & 5 \\
\hline
\hline
\end{tabular}
\tablebib{
(1) \cite{Vermeulen03}; (2) \cite{Maccagni17}; (3) \cite{Gupta06}; (4) \cite{Grasha19}; (5) \cite{Sanghera95}.
}
\tablefoot{
\small{
    Column\,1: Source name (J2000); Column\,2: Optical redshift; Columns\,3: Peak \hi\ 21-cm absorption redshift; Column\,4 - 5: Velocity to the bluer and redder side of the peak, respectively, where optical depth approaches zero; Column\,6: Flux density at 1.4 GHz; Column\,7: Radio luminosity at 1.4\,GHz; Column\,8: Flux density at the redhsifted 21-cm line frequency; Column\,9: Total velocity integrated optical depth; Column\,10: \hi\ 21-cm absorption reference; Column\,11: Largest Angular Size in arcsec, and Column\,12: Largest Linear Size in kpc; Column\,13: Reference for LAS and LLS.\\}
    \footnotesize{$^{\dag}$ measured with respect to $z_{em}$(opt).\\}
}
\end{sidewaystable*}
